Seeded Hierarchical Clustering for Expert-Crafted Taxonomies

Practitioners from many disciplines (e.g., political science) use expert-crafted taxonomies to make sense of large, unlabeled corpora. In this work, we study Seeded Hierarchical Clustering (SHC): the task of automatically fitting unlabeled data to such taxonomies using only a small set of labeled examples. We propose HierSeed, a novel weakly supervised algorithm for this task that uses only a small set of labeled seed examples. It is both data and computationally efficient. HierSeed assigns documents to topics by weighing document density against topic hierarchical structure. It outperforms both unsupervised and supervised baselines for the SHC task on three real-world datasets.

==> figs/overview.tex <==
\begin{figure}[tp]
\centering
\includegraphics[width=\linewidth]{methodOverview}
\caption{Overview of proposed algorithm. 
Step (3) (from Algorithm \ref{alg:shc}) corresponds to bottom-up update of topic representations (excluding leaf), up to pivot $\rho$.
$\delta_j$ is the core set assigned in step (6) using topic threshold.
Step (9, 12) corresponds to top-down assignment of all sets $\delta_x$ while updating topic representation (excluding level $\rho$). 
This process repeats until convergence. 
}
\label{tab:methodOverview}
\end{figure}

==> tables/level_stats.tex <==
\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ccccccccc}
	 \hline
	  & Level_1 & Level_2 & Level_3 & Level_4 & Level_5 & Level_6 & Level_7 & Level_8 \\
	 \hline
	 \hline
	 WOS & 6712 & 351 & - & - & - & -  & -  & - \\
	 NYT & 15161 & 2923 & 1160 & 842 & 1066 & 925  & 992  & 1460 \\
	 RCV1 & 236334 & 20523 & 11850 & 23211 & - & -  & -  & - \\
	 \hline
\end{tabular}%
}
\caption{\label{level_histogram}
The average number of occurrences of each topic at each level in the hierarchy.\emily{not sure we need this table}
}
\end{table}
